Optimal Search Trees with 2-Way Comparisons

In 1971, Knuth gave an $O(n^2)$-time algorithm for the classic problem of finding an optimal binary search tree. Knuth's algorithm works only for search trees based on 3-way comparisons, while most modern computers support only 2-way comparisons (e.g., $<, \le, =, \ge$, and $>$). Until this paper, the problem of finding an optimal search tree using 2-way comparisons remained open -- poly-time algorithms were known only for restricted variants. We solve the general case, giving (i) an $O(n^4)$-time algorithm and (ii) an $O(n \log n)$-time additive-3 approximation algorithm. Also, for finding optimal binary split trees, we (iii) obtain a linear speedup and (iv) prove some previous work incorrect.

==> huang1984.tex <==
\begin{verbatim}
#!/usr/bin/env python3.4

import sys
from functools import lru_cache
memoize = lru_cache(maxsize=None)

def huang1984(weights):
    n = len(weights)
    b = {i+1 : weights[key] for i,key in enumerate(sorted(weights.keys()))}

    def legal(i, j, d):
        return 0 <= i <= j <= n and 0 <= d <= j - i

    # return optimal cost p[i,j,d], weight w[i,j,d], and key set for t[i,j,d]
    @memoize
    def p_w_t(i, j, d):
        if d == j-i:            # lemma 3, or all keys deleted
            return 0, 0, set()

        def candidates():
            for k in range(i+1, j+1):
                for m in range(d+2):
                    if legal(i, k-1, m) and legal(k-1, j, d-m+1):
                        cost_l, weight_l, keys_l = p_w_t(i, k-1, m)
                        cost_r, weight_r, keys_r = p_w_t(k-1, j, d-m+1)
                        keys = keys_l | keys_r
                        deleted = set(range(i+1, j+1)) - keys
                        x = min(deleted, key = lambda h : b[h])
                        keys.add(x)
                        weight = b[x] + weight_l + weight_r
                        cost = weight + cost_l + cost_r
                        yield cost, weight, keys

        return min(candidates()) # lemma 4

    cost, weight, keys = p_w_t(0, n, 0)
    return cost

weights = dict(                               b4=20,
                        a3=20,                                         v3=20,
             a2=20,                 p2=20,                   t2=20,                 x2=20,
       a1=20,     d1=22,      n1=20,      q1=20,       s1=20,      u1=20,      w1=20,      y1=20,
    b0=9, c0=5, d0=9, e0=9, n0=9, p0=9, q0=9, r0=9,  s0=9, t0=9, u0=9, v0=9, w0=9, x0=9, y0=9, z0=9
)
cost1 = huang1984(weights)
print( cost1 )                  # 1688

weights['d1'] += 1
cost2 = huang1984(weights)
print( cost2 )                  # 1688, so algorithm must be wrong
\end{verbatim}

